Planet population synthesis driven by pebble accretion in cluster environments

The evolution of protoplanetary discs embedded in stellar clusters depends on the age and the stellar density in which they are embedded. Stellar clusters of young age and high stellar surface density destroy protoplanetary discs by external photoevaporation and stellar encounters. Here we consider the effect of background heating from newly formed stellar clusters on the structure of protoplanetary discs and how it affects the formation of planets in these discs. Our planet formation model is build on the core accretion scenario including pebble accretion. We synthesize planet populations that we compare to observations. The giant planets in our simulations migrate over large distances due to the fast type-II migration regime induced by a high disc viscosity ($\alpha=5.4 \times 10^{-3}$). Cold Jupiters (r>1 AU) originate preferably from the outer disc, while hot Jupiters (r<0.1 AU) preferably form in the inner disc. We find that the formation of gas giants via pebble accretion is in agreement with the metallicity correlation, meaning that more gas giants are formed at larger metallicity. However, our synthetic population of isolated stars host a significant amount of giant planets even at low metallicity, in contradiction to observations where giant planets are preferably found around high metallicity stars, indicating that pebble accretion is very efficient in the standard pebble accretion framework. On the other hand, discs around stars embedded in cluster environments hardly form any giant planets at low metallicity in agreement with observations, where these changes originate from the increased temperature in the outer parts of the disc, which prolongs the core accretion time-scale of the planet. We therefore conclude that the outer disc structure and the planet's formation location determines the giant planet occurrence rate and the formation efficiency of cold and hot Jupiters.

==> ucs.tex <==
%%
%% This is file `ucs.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ucs.dtx  (with options: `ucs.sty')
%% 
%% Copyright 2001 Dominique Unruh  <unruh@ut.ee>
%% Copyright 2013 Wolfgang Jeltsch <wolfgang@cs.ioc.ee>
%% 
%% This program is provided under the terms of the LaTeX Project Public License with some
%% modifications. See the file LICENSE for information.
%% 
\catcode`\@11
\ifx\@gobble\undefined\def\@gobble#1{}\fi
\ifx\@gobbletwo\undefined\def\@gobbletwo#1#2{}\fi
\ifx\@gobblethree\undefined\def\@gobblethree#1#2#3{}\fi
\ifx\@gobblefour\undefined\def\@gobblefour#1#2#3#4{}\fi
\ifx\@firstofone\undefined\def\@firstofone#1{#1}\fi
\ifx\@tempcnta\undefined\csname newcount\endcsname\@tempcnta\fi
\ifx\@tempcntb\undefined\csname newcount\endcsname\@tempcntb\fi
\ifx\@testopt\undefined
  \def\@testopt#1#2{%
    \@ifnextchar[{#1}{#1[{#2}]}}\fi
\ifx\@protected@testopt\undefined\def\@protected@testopt{\expandafter\@testopt\@gobble}\fi
\let\@let@token\relax
\ifx\@ifnextchar\undefined
  \def\@ifnextchar#1#2#3{%
    \let\reserved@d=#1%
    \def\reserved@a{#2}%
    \def\reserved@b{#3}%
    \futurelet\@let@token\@ifnch}\fi
\ifx\@ifnch\undefined
  \def\@ifnch{%
    \ifx\@let@token\@sptoken
      \let\reserved@c\@xifnch
    \else
      \ifx\@let@token\reserved@d
        \let\reserved@c\reserved@a
      \else
        \let\reserved@c\reserved@b
      \fi
    \fi
    \reserved@c}\fi
\ifx\@inputcheck\undefined\newread\@inputcheck\fi
\ifx\IfFileExists\undefined
\long\def\IfFileExists#1#2#3{%
  \openin\@inputcheck#1 %SPACE
  \ifeof\@inputcheck\def\reserved@a{#3}%
  \else\closein\@inputcheck\def\reserved@a{#2}%
  \fi
  \reserved@a}%
\fi
\ifx\InputIfFileExists\undefined
\long\def\InputIfFileExists#1#2{%
  \IfFileExists{#1}{#2\input #1 }}
\fi
\ifx\protect\undefined\let\protect\relax\fi
\ifx\@typeset@protect\undefined\let\@typeset@protect\relax\fi
\ifx\IeC\undefined\def\IeC{\ifx\protect\@typeset@protect
  \expandafter\@firstofone\else\noexpand\IeC\fi}\fi
\def\unicode@knownoptions{}
\def\XDeclareUnicodeOption#1#2#3#4#5{%
  \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse
  \expandafter\def\csname UnicodeOption#2true%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iftrue}%
  \expandafter\def\csname UnicodeOption#2false%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse}%
  \expandafter\def\csname @unicode@option@#2\endcsname{%
    #3\uni@activate@option{#2}{}{#4}{#5}}%
  \expandafter\def\csname @unicode@option@no#2\endcsname{%
    #3\uni@activate@option{#2}{no}{#4}{#5}}%
  \ifx~#1~\else\LinkUnicodeOptionToPkg{#2}{#1}\fi
  \let\uc@tempa\\\let\\\relax
  \edef\unicode@knownoptions{\\{#2}\unicode@knownoptions}%
  \let\\\uc@tempa
  }%
\let\uc@newcommand\def
\uc@newcommand\DeclareUnicodeOption{\@protected@testopt\DeclareUnicodeOption\DeclareUnicodeOption@{}}
\uc@newcommand\DeclareUnicodeOption@[#1]#2{%
  \XDeclareUnicodeOption{#1}{#2}{}{}{}}%
\uc@newcommand\uc@errormsg#1#2{%
  \ifx\PackageError\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \errhelp{#2}\errmessage{Package ucs: #1}}%
  \else
    \PackageError{ucs}{#1}{#2}%
  \fi
}%
\uc@newcommand\uc@warnmsg#1{%
  \ifx\PackageWarning\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \message{Package ucs: #1\MessageBreak}}%
  \else
    \PackageWarning{ucs}{#1}%
  \fi
}%
\def\uni@activate@option#1#2#3#4#5{%
  \ifx\uni@dataloaded\undefined
  \global\expandafter\def\csname @unicode@option@#1\endcsname##1{%
    \csname UnicodeOption#1true\endcsname
    \expandafter\def\csname uo-prio-#1\endcsname{##1}#3}%
  \global\expandafter\def\csname @unicode@option@no#1\endcsname##1%
    {\csname UnicodeOption#1false\endcsname#4}%
  \global\expandafter\let\csname uni@active@#1\endcsname1%
  \csname @unicode@option@#2#1\endcsname{#5}\else
  \uc@errormsg{Option #1 must be activated or deactivated %SPACE
    at least once in the preamble before using it in the document}{%
    For optimization causes I must know all %SPACE
    options before loading any unicode data.\MessageBreak
    Try e.g. #1 or no#1 as package option to ucs.}\fi}
\def\LinkUnicodeOptionToPkg#1#2{%
  \AtBeginDocument{\@ifpackageloaded{#2}{\SetUnicodeOption{#1}}{}}}%
\uc@newcommand\SetUnicodeOption{\@protected@testopt\SetUnicodeOption\SetUnicodeOption@{100}}
\uc@newcommand\SetUnicodeOption@[#1]#2{%
  \edef\uc@temp@a{@unicode@option@#2}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax
    \PackageError{ucs}{Unknown unicode option #2}{}%
  \else
    \csname\uc@temp@a\endcsname{#1}%
  \fi}
\ifx\ProvidesPackage\undefined\else
\ProvidesPackage{ucs}[2013/05/11 v2.2 UCS: Unicode input support]%
\fi
\ifx\@@input\undefined\input uni-global.def \else\input{uni-global.def}\fi
\DeclareUnicodeOption{fasterrors}
\DeclareUnicodeOption{warnunknown}
\DeclareUnicodeOption{graphics}
\DeclareUnicodeOption{savemem}
\DeclareUnicodeOption{document}
\SetUnicodeOption[1000]{document}
\DeclareUnicodeOption{default}
\SetUnicodeOption[0]{default}
\XDeclareUnicodeOption{}{combine}{}{%
  \let\uc@cmb\empty}{%
  \ifx\unicodecombine\undefined\else\unicodecombine\fi
  \def\uc@cmb{\uc@warn@nocombine}}%
\ifx\AtBeginDocument\undefined\else
  \AtEndDocument{\unicodecombine}\fi
\SetUnicodeOption{nocombine}%
\def\uc@cmb{\uc@warn@nocombine}%
\ifx\DeclareOption\undefined\else
\DeclareOption{showmagickern}{\def\uc@magic@glue{6805678}}%
\DeclareOption{hyperref}{\AtEndOfPackage{\RequirePackage{ucshyper}}}%
\DeclareOption*{\SetUnicodeOption{\CurrentOption}}\ProcessOptions*
\fi
\ifx\AtBeginDocument\undefined
  \uc@warnmsg{Not loading ucsencs.def automatically.\MessageBreak
    Please load it after initializing fontencodings}%
\else
  \AtBeginDocument{\input{ucsencs.def}}\fi
\AtBeginDocument{\ifUnicodeOptiongraphics\RequirePackage{graphicx}\fi}%
\uc@newcommand\unicode@numtohex{\protect\unicode@numtohex@}%
\uc@newcommand\unicode@numtohex@#1#2#3{%
  {%\let\empty\relax\relax
   %\ifx\empty\relax\def\empty{}%
     \count255=#2\relax\gdef#1{}%
     \count252=#3%
     \loop
     \count253=\count252\advance\count253by\count255\relax
     \ifnum\count253>0%
     \ifnum\count252>0\advance\count252by-1\relax\fi
     \count254=\count255%
     \divide\count255by16%
     \multiply\count255by16%
     \advance\count254by-\count255%
     \xdef#1{\ifcase\count254 0\or1\or2\or3\or4\or5\or6\or7\or
       8\or9\or A\or B\or C\or D\or E\or F\fi#1}%
     \divide\count255by16\relax
     \repeat
   %\else
   %  \def#1{dec:#2}%
   %\fi
   }}
\let\uc@spc\space
\newcount\uc@secondtry
\uc@newcommand\unicode@invalid#1{%
  \unicode@combine%
  \ifUnicodeOptiongraphics{%
  \ifx\unicode@graphicsdir\undefined
    \def\unicode@graphicsdir{ucs-glyphs}\fi
  \ifx\unicode@graphicscmd\undefined
    \def\unicode@graphicscmd{ucs-getglyph \hex\space \dec\space \path\space}\fi
  \unicode@numtohex\hex{#1}4%
  \count255=#1\relax
  \divide\count255 by256\relax
  \unicode@numtohex\uc@temp@b{\count255}2%
  \edef\path{\unicode@graphicsdir/\uc@temp@b/U\hex.ps}%
  \edef\dec{\number#1}%
  \IfFileExists{\uc@temp@c}{}{%
    \typeout{Running: \unicode@graphicscmd}%
    \immediate\write18{\unicode@graphicscmd}%
    }%
 \IfFileExists{\path}{%
    \setbox255=\hbox{X}%
    \edef\uc@temp@b{\begingroup\noexpand\uni@resetcatcodes
      \noexpand\includegraphics[height=\the\ht255, trim=0 22.5 0 17.5]%
                      {\path}%
    \noexpand\ProvidesFile{U\hex.ps}%
        [Downloaded glyph for U+\hex]%
    \endgroup}%
  \typeout{\meaning\uc@temp@b}%
  \expandafter\unicodevirtual\expandafter{\uc@temp@b}%
  }{%
    \PackageWarning{ucs}{File \uc@temp@d\uc@temp@c.ps %SPACE
      not found.\MessageBreak
      Use\MessageBreak
      \space\space\space\space\unicode@graphicscmd\MessageBreak
      or start latex with option -shell-escape\MessageBreak
      if you have not already done so.}%
    \unicodevirtual{\unicode@invalidglyph{#1}}}}\else
    \unicodevirtual{\unicode@invalidglyph{#1}}\fi}
\uc@newcommand\unicode@invalidglyph#1{%
  {\unicode@numtohex\uc@temp@d{#1}4%
    \fontencoding{OT1}\texttt{[U+\uc@temp@d]}}}
\uc@newcommand\uni@char#1{%
  \ucs@protected@unichar\iftrue
    \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
  %    \end{macrocode}
  % If the character is not defined yet, load it.
  %    \begin{macrocode}
      \begingroup
        % In case \let is not executed, this (until ===) expands
        % to \let\relax\relax,
        % otherwise we have \let\uc@notloaderr\@gobble
        % Number of \empty's must equal number of args of \uc@char@notloaded
        \let\uc@notloaderr\@gobble\empty\@gobbletwo\relax\relax
        % ===
      \expandafter\endgroup
      % If \let not executed: Warning is emitted (see |\uc@notloaderr|)
      % otherwise: |\uc@char@notloaded| is called.
      \uc@notloaderr{\number#1}\uc@char@notloaded{#1}%
    \else
  %    \end{macrocode}
  % If the character is loaded, run |\uc@checkopts|
  % with the options of this character
  % as first arg and the code position as second; this will
  % display the character with
  % the correct option.
  %    \begin{macrocode}
     \expandafter\expandafter\expandafter\uc@checkopts
       \expandafter\expandafter\expandafter
       {\csname u-\number#1-h/o\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\begingroup
  \lccode`\A=`\{\lccode`\B=`\}\lccode`\C=`\\%
  \lccode`\P=`\P\lccode`\U=`\U%
  \lowercase{%
\endgroup
  \uc@newcommand\uc@notloaderr#1#2#3{%
    \ifx\@gobble#1\else[Please insert %SPACE
      CPrerenderUnicodeACunicharA#1BB into preamble]\fi}}
\uc@newcommand\uc@checkopts#1#2{%
  \expandafter\uc@checkopt@error\expandafter{\number#2}%
    {error}{error}{infinity}#1\@nil
}
\expandafter\uc@newcommand\csname uo-prio-infinity\endcsname{-2100000000}
%% === BEGIN AUTOGENERATED CODE
\uc@newcommand\uc@checkopt@stick#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#2-#1\endcsname\relax
  \uc@localdeferr{#1}{#2}%
\else
  \uc@output{\csname u-#2-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#2\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#2\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#2}{#5}{#2}%
}
\uc@newcommand\uc@checkopt@change#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#3-#1\endcsname\relax
  \uc@localdeferr{#1}{#3}%
\else
  \uc@output{\csname u-#3-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#3\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#3\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#3}{#5}{#3}%
}
\uc@newcommand\uc@checkopt@error#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2, #3}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2, #3}{#5}{#4}%
}
\uc@newcommand\uc@checkopt@errorstick#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2}{#5}{#4}%
}
\let\unicode@empty\empty
\uc@newcommand\uc@errordrawopt#1#2#3{%
  \let\unicode@empty\relax\relax
  \ifx\unicode@empty\relax\let\unicode@empty\empty
    \unicode@numtohex\uc@temp@b{#1}4%
    \ifnum\csname uo-prio-#3\endcsname=-2100000000\relax
      \expandafter\ifx\csname
        missing-unicode-warned-\number#1\endcsname\relax
        \global\expandafter\let\csname
          missing-unicode-warned-\number#1\endcsname\@ne
        \unicode@error@unknown\@ne{Character \number#1\uc@spc
          \uc@spc= U+\uc@temp@b\uc@spc
          matches no activated options.\MessageBreak
          Type H to see available options}{#1}%
      \else
        \PackageWarning{ucs}{Character % SPACE
          \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
          appeared again.}%
      \fi
    \else
      \@getcharinfo\uc@temp@c{#1}%
      \PackageWarning{ucs}{Character %SPACE
        \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
        matches options\MessageBreak
        \uc@spc\uc@spc\uc@spc#2\MessageBreak
        with same priority \csname uo-prio-#3\endcsname. %SPACE
        Selecting option #3.\MessageBreak
        \uc@temp@c}%
      \uc@output{\csname u-#3-#1\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\uc@newcommand\uc@output#1#2{%
  \ifx\unicode@delay1\let\unicode@delay\relax\else
    \ifUnicodeOptioncombine
      \expandafter\uc@combine\expandafter{#1}{#2}%
    \else
      \uc@prechar@exec{#2}%
        \unicode@charfilter{#1{}}%
    \fi
    \ifx\uc@throw\undefined\else
      \def\uc@got{#2}\uc@throw\global\let\uc@throw\undefined\fi
  \fi
}%
\uc@newcommand\uc@prechar@exec#1{%
  \ifx\uc@prechar\undefined\else\uc@prechar{#1}\fi}
\uc@newcommand\uc@localdeferr#1#2{%
  \@getcharinfo\uc@temp@a{#1}%
  \PackageError{ucs}{Internal error in character \number#1, %SPACE
    option #2}{I probably got confused by intermixed local %SPACE
    and global definitions.\MessageBreak Try to load the needed %SPACE
    code page via \noexpand\PreloadUnicodePage
    before declaring anything by yourself.}{\uc@temp@a}%
  \unicode@invalid{#1}%
}%
\uc@newcommand\uc@warn@nocombine{%
  \PackageError{ucs}{Please activate option 'combine'}{Composed %SPACE
    characters can only be rendered correctly, when the option %SPACE
    'combine' is activated}}
\newtoks\uc@combtoks
\newtoks\uc@combtoksb
\newtoks\uc@temptokena
\uc@newcommand\unicode@combine{%
  \uc@check@magicglue%
  \ifx\uc@combining@prechar\undefined\global\let\uc@comb@code\undefined\fi
  \ifx\uc@comb@code\undefined\uc@temptokena{}\else
    \uc@temptokena\expandafter{\expandafter\uc@prechar@exec
      \expandafter{\uc@comb@code}}\fi%
  \global\let\uc@comb@code\undefined
  \global\expandafter\expandafter\expandafter\expandafter\expandafter
  \expandafter\expandafter\uc@combtoksb
  \expandafter\expandafter\expandafter
  \expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\the
    \expandafter\expandafter\expandafter\uc@combtoksb
    \expandafter\the\expandafter\uc@temptokena\the\uc@combtoks}%
  \global\uc@combtoks{}}
\def\uc@magic@glue{5381}
\uc@newcommand\uc@check@magicglue{%
  \ifnum\lastskip=\uc@magic@glue\unskip\else
    \begingroup
      \edef\uc@temp@a{\the\uc@combtoks}%
      \ifx\uc@temp@a\empty\else
      \PackageWarning{ucs}{Magic kern expected. Probably some %SPACE
        non-unicode characters mixed in while option combine was %SPACE
        in effect.}\fi\endgroup
  \fi}
\uc@newcommand\unicodevirtual#1{%
  \def\uc@temp@a##1{#1}\uc@output{\csname uc@temp@a\endcsname}{"FFFF}}
\uc@newcommand\unicodecombine{%
  \ifx\protect\@typeset@protect
    \unicode@combine%
    %\typeout{WRITING: \the\uc@combtoksb}%
    \the\uc@combtoksb
    \uc@prechar@exec{-1}%
    \global\uc@combtoksb{}%
      \ifx\uc@throw\undefined\else
        \def\uc@got{-1}\uc@throw\global\let\uc@throw\undefined\fi
  \else
    \noexpand\unicodecombine\fi
}
\uc@newcommand\uc@combine#1#2{%
  \ifx\protect\@typeset@protect
    \@temptokena\expandafter{#1{}}%
    \expandafter\expandafter\expandafter\ifx
    \expandafter\uc@firstofmany\the\@temptokena\uc@firstofmany\uc@cmb
      \uc@check@magicglue%
      \uc@combtoks\expandafter\expandafter\expandafter\expandafter
     \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter\@gobble
        \expandafter#1\expandafter{\the\uc@combtoks}}%
    \else
      \unicode@combine%
      \xdef\uc@comb@code{\number#2}%
      \global\uc@combtoks\expandafter{#1{}}%
    \fi
    %\typeout{->COMBTOKS: \the\uc@combtoks}%
    \hskip\uc@magic@glue spplus0ptminus0pt %SPACE ; Insert magic glue
  \else
    \noexpand\unichar{\number#2}\fi
}
\uc@newcommand\uc@char@notloaded#1{%
  \count255=#1\divide\count255 by 256%
  \edef\uc@temp@a{uni-\number\count255.def}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax\else
    \uc@secondtry#1\relax\fi
  \ifnum\uc@secondtry=#1\relax
    % If the file has already been loaded, but the character is unknown,
    % output an error and show the replacement glyph
    \unicode@numtohex\uc@temp@b{#1}4%
    \expandafter\ifx\csname
      missing-unicode-warned-\number#1\endcsname\relax
    \global\expandafter\let\csname
      missing-unicode-warned-\number#1\endcsname\@ne
      \unicode@error@unknown\@ne{Unknown Unicode character % SPACE
        \number#1 \uc@spc= U+\uc@temp@b,\MessageBreak
        possibly declared in \uc@temp@a.\MessageBreak
        Type H to see if it is available with options}{#1}%
    \else
      \PackageWarning{ucs}{Unknown character % SPACE
        \number#1 \uc@spc = 0x\uc@temp@b\uc@spc
        appeared again.}%
      \unicode@invalid{#1}%
    \fi
  \else
    \begingroup
    \ifUnicodeOptionsavemem
    \else
      \global\expandafter\let\csname\uc@temp@a\endcsname\@ne
    \fi
    \def\uc@got{#1}%
    \uni@resetcatcodes
    \expandafter\InputIfFileExists\expandafter{\uc@temp@a}{%
      \global\let\uni@dataloaded1%
      }{%
      }%
      % End of local group for inputted file
    \endgroup
      % Retry displaying character. This won't cause infinite recursion,
      % because we have marked this file as loaded (globally or, if
      % |savemem| is set, at least here).
    \uc@secondtry#1\relax%
    \uni@char{#1}%
  \fi
  }
\uc@newcommand\PreloadUnicodePage#1{%
  \begingroup
  \global\expandafter\let\csname uni-#1.def\endcsname\@ne
  \uni@resetcatcodes
  \InputIfFileExists{uni-#1.def}{\let\uni@dataloaded1}{%
    \PackageError{ucs}{Could not find uni-#1.def}{}}%
  \endgroup}
\uc@newcommand\PrerenderUnicode{%
  \@ifstar{\@prerenderunicode\unichar}{\@prerenderunicode\@gobble}}%
\uc@newcommand\@prerenderunicode#1#2{%
  \begingroup
  \UnicodeCharFilter\@gobble
  \let#1\@gobble\setbox0\hbox{#2}\endgroup}
\uc@newcommand\DeclareUnicodeCharacter#1#2{%
  \DeclareUnicodeCharacterAsOptional{#1}{document}{#2}}
\uc@newcommand\DeclareUnicodeCharacterAsOptional{%
  \let\uc@temp@a\relax\uni@declcharopt}
\uc@newcommand\uc@dclc#1#2{%
  \let\next=\uni@declcharopt
  \ifUnicodeOptionsavemem
    \ifnum\uc@got=#1\else
      \let\next=\@gobblethree\fi
  \fi
  \ifx\next\uni@declcharopt
    \expandafter\ifx\csname uni@active@#2\endcsname\relax
      \let\next\@gobblethree\else
    \expandafter\ifx\csname u-#2-\number#1\endcsname\relax\else
      \let\next\@gobblethree\fi\fi
    \let\uc@temp@a\global
  \fi
  \next{#1}{#2}}
\uc@newcommand\uni@declcharopt#1#2#3{%
  %\typeout{Defining: u-#2-\number#1 (\meaning\uc@temp@a)}%
  \ifx\utf@viii@map\undefined\else
    \expandafter\utf@viii@map\expandafter{\number#1}\fi
  \expandafter\uc@temp@a\expandafter\def
    \csname u-#2-\number#1\endcsname##1{#3}%\fi
  \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
    \expandafter\def\csname u-\number#1-h/o\endcsname{}\fi
  \expandafter\uc@temp@a\expandafter\edef
    \csname u-\number#1-h/o\endcsname{%
    {#2}\csname u-\number#1-h/o\endcsname}%
  }%
\let\unichar\uni@char
\uc@newcommand\unicodesuper#1{\textsuperscript{#1}}%
\uc@newcommand\@getcharinfo#1#2{%
  \begingroup
  \countdef\uc@got0\relax\uc@got#2\relax
  \global\def#1{Character's name unknown}%
  \def\info##1{\xdef#1{##1}}%
  \uni@resetcatcodes
  \ifUnicodeOptionfasterrors
  \global\def#1{No further informations known % SPACE
    because of option fasterrors.}\else
  {\InputIfFileExists{uninames.dat}{}{%
    \global\def#1{Character database uninames.dat not found. %SPACE
      \MessageBreak Character \number#2 \uc@spc unknown}}}%
  \fi
  \toks255{}%
  \def\uc@dclc##1##2##3{\ifnum##1=\uc@got
    \toks255\expandafter{\the\toks255, ##2}\fi}%
  \count255\uc@got\divide\count255by256\relax
  %\edef\temp@a{uni-\number\count255.def}%
  \InputIfFileExists{uni-\number\count255.def}{}{}%
  \expandafter\ifx\expandafter\@nil\the\toks255 \@nil
    \xdef#1{#1\noexpand\MessageBreak
      Character is not defined in uni-*.def files}%
  \else
    \expandafter\expandafter\expandafter\@getcharinfo@
    \expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter
    {\expandafter#1\expandafter}\the\toks255 \@nil%
  \fi
  \endgroup}
\def\@getcharinfo@#1#2, #3\@nil{\gdef#1{#2\MessageBreak
    Character available with following options:\MessageBreak
    \uc@spc\uc@spc\uc@spc #3}}
\uc@newcommand\PrintUnicodeName#1{{%
  \@getcharinfo{\ci}{#1}%
  \def\MessageBreak{^^J}%
  \typeout{^^J\ci^^J}}}
\uc@newcommand\UnicodeCharFilter#1{\let\unicode@charfilter=#1}
\uc@newcommand\UCSProtectionNone{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\@firstofone}
\uc@newcommand\UCSProtectionIeC{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\IeC}
\uc@newcommand\UCSProtectionUnichar{%
  \def\ucs@protected@unichar##1{\ifx\protect\@typeset@protect}%
  \UnicodeCharFilter\@firstofone}
\UCSProtectionIeC
\uc@newcommand\uni@resetcatcodes{%
  \endlinechar=13\relax
  \def\reserved@a##1##2{%
    \@tempcnta##1\relax
    \@tempcntb##2\relax
    \reserved@b
    }%
  \def\reserved@b{%
    \ifnum\@tempcnta>\@tempcntb\else
    \reserved@c\@tempcnta
    \advance\@tempcnta\@ne
    \expandafter\reserved@b
    \fi
    }%
  \catcode`\ =10\relax
  \catcode`\#=6\relax
  \catcode`\$=3\relax
  \catcode`\%=14\relax
  \catcode`\&=4\relax
  \catcode`\\=0\relax
  \catcode`\^=7\relax
  \catcode`\_=8\relax
  \catcode`\{=1\relax
  \catcode`\}=2\relax
  \catcode`\~=13\relax
  \catcode`\@=11\relax
  \catcode`\^^I=10\relax
  \catcode`\^^J=12\relax
  \catcode`\^^L=12\relax
  \catcode`\^^M=5\relax
  \def\reserved@c##1{\catcode##1=12\relax}%
  \reserved@c{`\!}%
  \reserved@c{`\"}%
  \reserved@a{`\'}{`\?}%
  \reserved@c{`\[}%
  \reserved@c{`\]}%
  \reserved@c{`\`}%
  \reserved@c{`\|}%
  \def\reserved@c##1{\catcode##1=11\relax}%
  \reserved@a{`\A}{`\Z}%
  \reserved@a{`\a}{`\z}%
  \def\reserved@c##1{\catcode##1=15\relax}%
  \reserved@a{0}{`\^^H}%
  \reserved@c{`\^^K}%
  \reserved@a{`\^^N}{31}%
  \catcode"7F=15\relax
  \relax}
\catcode`\!13\relax
\uc@newcommand\unicode@error@unknown{\protect\unicode@error@unknown@}%
\uc@newcommand\unicode@error@unknown@#1#2#3{%
  {\expandafter\countdef\expandafter\uc@got\expandafter0%
     \expandafter\relax\expandafter\uc@got\number#3\relax
  \ifx\measuring@false\undefined\else\measuring@false\fi
  \@getcharinfo\uc@temp@c{#3}%
  \ifUnicodeOptionwarnunknown
    \PackageWarning{ucs}{#2\MessageBreak\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne\unicode@invalid{#3}\fi
  \else
    \let!\unicode@read@definition\catcode`\!13\relax
    \let\uc@read@definition\undefined
    \PackageError{ucs}{#2}{\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne
    \ifx\uc@read@definition\undefined\unicode@invalid{#3}%
    \else\uc@read@definition\fi\fi
  \fi}}
\catcode`\!12\relax
\uc@newcommand\unicode@read@definition{%
  \uni@resetcatcodes
  \typein[\definition]{Please enter definition for %SPACE
    unicode character \number\uc@got}%
  \global\let\uc@read@definition\definition
  \toks255\expandafter{\definition}%
  \edef\definition{\noexpand\DeclareUnicodeCharacter%
    {\number\uc@got}{\the\toks255}}%
  \toks255\expandafter{\definition}%
  \typeout{Tip:\MessageBreak You may include\MessageBreak
    \uc@spc\uc@spc\the\toks255\MessageBreak
    into your document source.}%
  \the\toks255\relax
  }
\def\uc@firstofmany#1#2\uc@firstofmany{#1}
\ifx\AtBeginDocument\undefined\else
\AtBeginDocument{\def\uc@tempa{\@inpenc@undefined@{utf8}}%
  \ifx\@inpenc@undefined\uc@tempa
  \ifx\restore@utf@viii@actives\undefined
  \PackageWarning{ucs}{***************************\MessageBreak You %SPACE
    seem to have loaded inputencoding utf8\MessageBreak (LaTeX kernel %SPACE
    UTF-8) instead of utf8x (ucs.sty UTF-8).\MessageBreak Probably you %SPACE
    are compiling a document written for a\MessageBreak
    pre-august-2004 ucs.sty.\MessageBreak
    ***************************\MessageBreak Please use %SPACE
    \string\usepackage[utf8x]{inputenc} instead of\MessageBreak
    \string\usepackage[utf8]{inputenc}.\MessageBreak
    ***************************\MessageBreak If you should really want %SPACE
    to use ucs.sty and kernel's\MessageBreak utf8.def together, use %SPACE
    \string\usepackage[utf8x,utf8]{inputenc}\MessageBreak to disable %SPACE
    compatibility mode\MessageBreak
    ***************************\MessageBreak Activating compatibility %SPACE
    mode.\MessageBreak ***************************\MessageBreak}%
  \global\let\uc@inputencoding\inputencoding
  \inputencoding{utf8x}%
  \def\inputencoding#1{%
    {\def\uc@tempa{#1}\def\uc@tempb{utf8}\ifx\uc@tempa\uc@tempb
      \aftergroup\@firstoftwo\else\aftergroup\@secondoftwo\fi}%
    {\restore@utf@viii@actives}{\uc@inputencoding{#1}}}%
  \fi\fi
}\fi

